CodeAttack: Code-Based Adversarial Attacks for Pre-trained Programming Language Models

Pre-trained programming language (PL) models (such as CodeT5, CodeBERT, GraphCodeBERT, etc.,) have the potential to automate software engineering tasks involving code understanding and code generation. However, these models operate in the natural channel of code, i.e., they are primarily concerned with the human understanding of the code. They are not robust to changes in the input and thus, are potentially susceptible to adversarial attacks in the natural channel. We propose, CodeAttack, a simple yet effective black-box attack model that uses code structure to generate effective, efficient, and imperceptible adversarial code samples and demonstrates the vulnerabilities of the state-of-the-art PL models to code-specific adversarial attacks. We evaluate the transferability of CodeAttack on several code-code (translation and repair) and code-NL (summarization) tasks across different programming languages. CodeAttack outperforms state-of-the-art adversarial NLP attack models to achieve the best overall drop in performance while being more efficient, imperceptible, consistent, and fluent. The code can be found at https://github.com/reddy-lab-code-research/CodeAttack.

==> tables/results/quality.tex <==
\begin{table*}[h]
    \small
    \centering
    \begin{tabular*}{\textwidth}{p{4cm}|p{4cm}|p{4cm}|p{4cm}}
    \cline{1-4}
    \textbf{Original Code} & \tb{TextFooler} & \tb{BERT-Attack} & \tb{\model} \\
    \cline{1-4}
\cline{1-4}
\begin{C}[style=CStyle,basicstyle=\tiny]
public override void WriteByte(byte b) {
  if (outerInstance.upto == outerInstance.blockSize) {... }}
\end{C}&
\begin{C}[style=CStyle,basicstyle=\tiny]
<@\textcolor{red}{\tb{\hl{audiences revoked canceling}}}@> WriteByte(byte b) {
  if (outerInstance.upto == outerInstance.blockSize) {.... }}
\end{C}
& 
\begin{C}[style=CStyle,basicstyle=\tiny]
public override void<@\textcolor{red}{\tb{\hl{ ; .}}}@> b) {
  if (outerInstance.upto == outerInstance.blockSize) {... }}
\end{C}&
\begin{C}[style=CStyle,basicstyle=\tiny]
public override void WriteByte(<@\textcolor{red}{\tb{\hl{bytes}}}@> b) {
  if (outerInstance.upto == outerInstance.blockSize) {... }}
\end{C}\\
\tiny{CodeBLEU$_\textnormal{before}$:100} & \tiny{$\Delta_{drop}$:5.74; \qquad CodeBLEU$_q$: 63.28} & \tiny{$\Delta_{drop}$:27.26; \qquad CodeBLEU$_q$:49.87} & \tiny{$\Delta_{drop}$:20.04;\qquad CodeBLEU$_q$: 91.69}\\
\cline{1-4}
    \end{tabular*}
    \caption{Qualitative examples of adversarial codes on C\#-Java Code Translation task. (See Appendix A for more examples).}
    \label{tab:qual}
\end{table*}


